Robust Unsupervised StyleGAN Image Restoration

GAN-based image restoration inverts the generative process to repair images corrupted by known degradations. Existing unsupervised methods must be carefully tuned for each task and degradation level. In this work, we make StyleGAN image restoration robust: a single set of hyperparameters works across a wide range of degradation levels. This makes it possible to handle combinations of several degradations, without the need to retune. Our proposed approach relies on a 3-phase progressive latent space extension and a conservative optimizer, which avoids the need for any additional regularization terms. Extensive experiments demonstrate robustness on inpainting, upsampling, denoising, and deartifacting at varying degradations levels, outperforming other StyleGAN-based inversion techniques. Our approach also favorably compares to diffusion-based restoration by yielding much more realistic inversion results. Code is available at https://lvsn.github.io/RobustUnsupervised/.

==> conclusion.tex <==
\section{Conclusion}
We have shown that a few key changes suffice to make StyleGAN image restoration robust to both variability in degradation levels and to compositions of different degradations. Our proposed method still relies on two strong assumptions: (approximate) knowledge of the degradation function used, and domain-specificity of the generative model. Relaxing both assumptions is of great interest and some headway has already been made in parallel work.
